Coalesced Matrix-Free Finite Elements in Cell-Wise Storage

We present a GPU-oriented formulation of continuous high-order finite elements in which the redundant, cell-wise (element-local) vector is the persistent primary representation of all field data, rather than a transient stage of matrix-free operator evaluation. We prove that, given a preconditioner whose image is continuous, the entire flexible conjugate gradient iteration can be carried out exactly on this unassembled representation: a simple primal-dual pairing identity shows that all Krylov scalars computed from local data coincide with those of the assembled solve, so inter-element communication is confined entirely to the preconditioner. The required direct stiffness summation (DSS) is then realized without indirect gather-scatter, atomics, or coloring, by a dimensionally-split cascade of one-to-one face exchanges that provably accumulates edge and vertex contributions as a byproduct of sequential axis passes; unstructured macro-block interfaces and $h$-adaptive hanging nodes are handled by disjoint topological kernels and a shadow-cell wrapper that leaves the high-throughput sweeps untouched. The cell-wise storage decouples the memory layout from the mesh topology, and we exploit this freedom to benchmark blocked layouts that trade memory coalescing against element contiguity. Numerical experiments on modern GPUs demonstrate that the resulting operator evaluation and solver outperform state-of-the-art matrix-free implementations, signifficantly exceeding throughput of existing implementations.

==> figures/fig_mg_convergence.tex <==
% V-cycle convergence of the DSS multigrid solver, fp64. MG only (no CG).
% Two panels: (a) uniform refinement, (b) adaptive refinement with hanging
% nodes. Both [REAL DATA].
% x = V-cycle index, y = residual measure (eq:energy_measure defines
% energy = sqrt(<r,u>); we plot <r,u> itself, i.e. the energy measure squared).
% Solid lines: energy measure <r,u> (squared, sqrt not taken); dashed
% lines: ||sync(r)|| as-is (already a plain norm, not squared), the Euclidean
% norm of the DSS-synchronized residual (only meaningful on the
% uniform/conforming mesh of panel (a)).
% One colour per polynomial degree (p = 2, 3, 4).
%
% Panel (a) data: raw_results/multigrid/mg_convergence.csv, generated by
%   raw_results/multigrid/parse_convergence.py from
%   raw_results/multigrid/sweep_cube_monitor_smooth2.out (solver=mg, REF=8).
% Panel (b) data: raw_results/multigrid/mg_convergence_adaptive.csv, generated
%   by raw_results/multigrid/parse_convergence.py from
%   raw_results/multigrid/sweep_cube_adaptive_smooth2_monitor.out
%   (solver=mg, global=5, adaptive=4).
%
% This file provides the two subfigures; the outer figure environment with the
% overall caption/label lives in splitted/multigrid.tex.
\pgfplotsset{
    mgconv/.style={
            width=\linewidth, height=0.85\linewidth,
            xlabel={V-cycle}, ylabel={residual measure},
            xmin=0, xmax=19, ymin=1e-20, ymax=1,
            grid=both,
            legend style={font=\scriptsize, at={(0.97,0.97)}, anchor=north east},
            legend columns=1, legend cell align=left,
        },
}
\begin{subfigure}[b]{0.49\linewidth}
    \centering
    \begin{tikzpicture}
        \begin{semilogyaxis}[mgconv]
            \addplot[orange, mark=square*,   thick, opacity=0.55]  table[col sep=comma, x=cycle, y=p2_energy_sq] {raw_results/multigrid/mg_convergence.csv};
            \addplot[orange, mark=square,    dashed, mark options={solid}, forget plot] table[col sep=comma, x=cycle, y=p2_sync]   {raw_results/multigrid/mg_convergence.csv};
            \addplot[teal,   mark=triangle*, thick, opacity=0.55]  table[col sep=comma, x=cycle, y=p3_energy_sq] {raw_results/multigrid/mg_convergence.csv};
            \addplot[teal,   mark=triangle,  dashed, mark options={solid}, forget plot] table[col sep=comma, x=cycle, y=p3_sync]   {raw_results/multigrid/mg_convergence.csv};
            \addplot[blue,   mark=diamond*,  thick, opacity=0.55]  table[col sep=comma, x=cycle, y=p4_energy_sq] {raw_results/multigrid/mg_convergence.csv};
            \addplot[blue,   mark=diamond,   dashed, mark options={solid}, forget plot] table[col sep=comma, x=cycle, y=p4_sync]   {raw_results/multigrid/mg_convergence.csv};
            \legend{$p{=}2$, $p{=}3$, $p{=}4$}
        \end{semilogyaxis}
    \end{tikzpicture}
    \caption{Uniform refinement.}
    \label{fig:mg_conv_uniform}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\linewidth}
    \centering
    \begin{tikzpicture}
        \begin{semilogyaxis}[mgconv]
            \addplot[orange, mark=square*,   thick, opacity=0.55]  table[col sep=comma, x=cycle, y=p2_energy_sq] {raw_results/multigrid/mg_convergence_adaptive.csv};
            \addplot[orange, mark=square,    dashed, mark options={solid}, forget plot] table[col sep=comma, x=cycle, y=p2_sync]   {raw_results/multigrid/mg_convergence_adaptive.csv};
            \addplot[teal,   mark=triangle*, thick, opacity=0.55]  table[col sep=comma, x=cycle, y=p3_energy_sq] {raw_results/multigrid/mg_convergence_adaptive.csv};
            \addplot[teal,   mark=triangle,  dashed, mark options={solid}, forget plot] table[col sep=comma, x=cycle, y=p3_sync]   {raw_results/multigrid/mg_convergence_adaptive.csv};
            \addplot[blue,   mark=diamond*,  thick, opacity=0.55]  table[col sep=comma, x=cycle, y=p4_energy_sq] {raw_results/multigrid/mg_convergence_adaptive.csv};
            \addplot[blue,   mark=diamond,   dashed, mark options={solid}, forget plot] table[col sep=comma, x=cycle, y=p4_sync]   {raw_results/multigrid/mg_convergence_adaptive.csv};
            \legend{$p{=}2$, $p{=}3$, $p{=}4$}
        \end{semilogyaxis}
    \end{tikzpicture}
    \caption{Adaptive refinement with hanging nodes.}
    \label{fig:mg_conv_adaptive}
\end{subfigure}


==> figures/fig_mg_roofline.tex <==
% Roofline of the multigrid building blocks on the A100 80GB SXM (FP64).
% Four kernel families: operator evaluation (Laplace apply), restriction,
% prolongation, and the cell-wise smoother.
% Each family has one point per polynomial degree p = 2..5, connected by a line.
% All are memory bound, so the points cluster near the bandwidth slope.
% Two panels: (left) general geometry, (right) Cartesian geometry.
% Transfers (restriction + prolongation) are geometry-independent and identical
%   in both panels (sweep_transf_profile). Operator eval + smoother differ:
%   left panel from sweep_cube_profile2 (Cartesian), right from sweep_ball_profile
%   (general).
%
% Reusable axis style shared by both panels.
\pgfplotsset{
    mg roofline axis/.style={
            width=\linewidth,
            height=0.8\linewidth,
            xlabel={Arithmetic intensity [FLOP/byte]},
            ylabel={Performance [TFLOP/s]},
            log basis x=2,
            xmin=0.25, xmax=16,
            xtick={0.25,0.5,1,2,4,8,16},
            xticklabels={$\frac{1}{4}$,$\frac{1}{2}$,1,2,4,8,16},
            log basis y=2,
            ymin=0.5, ymax=32,
            ytick={0.5,1,2,4,8,16,32},
            yticklabels={$\frac{1}{2}$,1,2,4,8,16,32},
            grid=both,
            legend cell align=left,
            % Common horizontal legend, captured once (on the left panel) and
            % printed above both panels; see \ref{mgrooflinelegend} below.
            legend columns=-1, legend style={/tikz/every even column/.append style={column sep=1em}}, }, }
%
% Rooflines + memory-bound/compute-bound regions, shared by both panels.
\newcommand{\mgrooflinebackground}{%
    % --- Colored regions ---
    % Outer corners are pushed far outside any plausible axis range; only the
    % diagonal boundary points (bandwidth line meets 9.7 at x=4.76 and 19.5 at
    % x=9.56) are physical. pgfplots clips to the axis box, so the same macro
    % renders correctly regardless of each panel's xmin/xmax/ymin/ymax.
    \addplot[green, fill=green, draw=none, fill opacity=0.3, forget plot]
    coordinates {(0.001,0.002039) (4.76,9.7) (1000,9.7) (1000,0.0001) (0.001,0.0001)};
    \addplot[cyan, fill=cyan, draw=none, fill opacity=0.3, forget plot]
    coordinates {(4.76,9.7) (9.56,19.5) (1000,19.5) (1000,9.7)};
    % --- Rooflines: A100 80GB SXM (FP64), bandwidth 2039 GB/s ---
    \addplot[thick, domain=0.001:9.56, samples=2, forget plot] {2.039*x};
    \addplot[thick, domain=0.001:1000, samples=2, forget plot] {9.7};
    \addplot[thick, dashed, domain=0.001:1000, samples=2, forget plot] {19.5};
}
%
% Roofline labels (left panel only). Pinned to fixed data coordinates.
\newcommand{\mgrooflinelabels}{%
    \node[rotate=37.4, above, font=\small\bfseries] at (axis cs:1.2,2.2) {Bandwidth 2039 GB/s};
    \node[above right, font=\small\bfseries] at (axis cs:0.26,9.7) {CUDA 9.7 TFLOP/s};
    \node[above right, font=\small\bfseries] at (axis cs:0.26,19.5) {Tensor 19.5 TFLOP/s};
}
%
% Transfers (geometry-independent), shared by both panels.
\newcommand{\mgrooflinetransfers}{%
    % Restriction (measured, sweep_transf_profile)
    \addplot[red, mark=square*, mark size=2.5pt, thick]
    coordinates {(0.079,0.122) (1.714,2.117) (1.745,1.784) (1.430,1.507)};    % p=2,3,4,5
    \addlegendentry{Restriction}
    % Prolongation (measured, sweep_transf_profile)
    \addplot[orange, mark=diamond*, mark size=2.5pt, thick]
    coordinates {(0.583,0.981) (0.888,1.445) (1.587,2.423) (1.567,2.183)};    % p=2,3,4,5
    \addlegendentry{Prolongation}
}
%
% Common horizontal legend, printed above both panels.
\begin{center}
    \ref{mgrooflinelegend}
\end{center}
%
\begin{subfigure}{0.49\linewidth}
    \centering
    \begin{tikzpicture}
        \begin{loglogaxis}[mg roofline axis, legend to name=mgrooflinelegend]
            \mgrooflinebackground
            \mgrooflinelabels
            % --- Operator evaluation + smoother (Cartesian, sweep_cube_profile2) ---
            \addplot[black, mark=*, mark size=2.5pt, thick]
            coordinates {(2.167,3.518) (5.436,7.503) (6.895,7.245) (6.707,5.711)};      % p=2,3,4,5
            \addlegendentry{Operator eval.}
            \mgrooflinetransfers
            \addplot[blue, mark=triangle*, mark size=2.5pt, thick]
            coordinates {(0.460,0.689) (1.160,1.803) (1.496,1.753) (1.489,1.676)};      % p=2,3,4,5
            \addlegendentry{Smoother}
        \end{loglogaxis}
    \end{tikzpicture}
    \caption{Cartesian geometry}\label{fig:mg_roofline_cartesian}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
    \centering
    \begin{tikzpicture}
        \begin{loglogaxis}[mg roofline axis, legend to name=mgrooflinelegendunused,
                % General geometry sits low, so drop the axis floor to show all
                % transfer points (incl. the p=2 restriction outlier).
                xmin=0.0625, xtick={0.0625,0.125,0.25,0.5,1,2,4,8,16},
                xticklabels={$\frac{1}{16}$,$\frac{1}{8}$,$\frac{1}{4}$,$\frac{1}{2}$,1,2,4,8,16},
                ymin=0.0625, ytick={0.0625,0.125,0.25,0.5,1,2,4,8,16,32},
                yticklabels={$\frac{1}{16}$,$\frac{1}{8}$,$\frac{1}{4}$,$\frac{1}{2}$,1,2,4,8,16,32}]
            \mgrooflinebackground
            % --- Operator evaluation + smoother (general geometry, sweep_ball_profile) ---
            \addplot[black, mark=*, mark size=2.5pt, thick]
            coordinates {(0.228,0.358) (1.026,1.541) (1.103,1.606) (1.046,1.517)};      % p=2,3,4,5
            \addlegendentry{Operator eval.}
            \mgrooflinetransfers
            \addplot[blue, mark=triangle*, mark size=2.5pt, thick]
            coordinates {(0.211,0.324) (0.839,1.243) (0.922,1.286) (0.888,1.233)};      % p=2,3,4,5
            \addlegendentry{Smoother}
        \end{loglogaxis}
    \end{tikzpicture}
    \caption{General geometry}\label{fig:mg_roofline_general}
\end{subfigure}


==> tables/tab_mg_adaptive_iters.tex <==
% CG iteration count vs. number of adaptive refinements (refinement independence).
% Data: raw_results/multigrid/sweep_{cube,ball}_adaptive_smooth2.out
%   (2 smoothing steps). Smallest global refinement in the sweep (global = 5)
%   is used so that the adaptive levels 1..4 are the only varying quantity.
% Values are the CG iteration count to the fixed energy-norm reduction with the
% DSS multigrid as preconditioner. A dash (--) marks a run absent from the sweep.
% Ball p=1 omitted (CG hit the 20-iteration cap without converging).
\subcaptionbox{Cube\label{tab:mg_adaptive_iters_cube}}{%
    \begin{tabular}{@{}c*{4}{>{\centering\arraybackslash}p{2.4em}}@{}}
        \toprule
            & \multicolumn{4}{c}{Adaptive refinements}                   \\
        \cmidrule(lr){2-5}
        $p$ & $1$                                      & $2$ & $3$ & $4$ \\
        \midrule
        $2$ & 9                                        & 10  & 9   & 9   \\
        $3$ & 10                                       & 10  & 10  & 10  \\
        $4$ & 10                                       & 10  & 10  & 10  \\
        $5$ & 11                                       & 12  & 12  & 12  \\
        \bottomrule
    \end{tabular}}
\qquad\qquad
\subcaptionbox{Ball\label{tab:mg_adaptive_iters_ball}}{%
    \begin{tabular}{@{}c*{4}{>{\centering\arraybackslash}p{2.4em}}@{}}
        \toprule
            & \multicolumn{4}{c}{Adaptive refinements}                   \\
        \cmidrule(lr){2-5}
        $p$ & $1$                                      & $2$ & $3$ & $4$ \\
        \midrule
        $2$ & 12                                       & 13  & 13  & 13  \\
        $3$ & 14                                       & 14  & 14  & 14  \\
        $4$ & 14                                       & 14  & 14  & --  \\
        \bottomrule
    \end{tabular}}


==> tables/tab_mg_adaptive_solve_time.tex <==
% Solve-time comparison of the DSS multigrid on adaptively refined meshes.
% Data: raw_results/multigrid/sweep_{cube,ball}_adaptive_smooth2.out
%   (2 smoothing steps). Highest adaptive-refinement level in the sweep
%   (adaptive = 4) is used, at the highest global refinement with completed
%   runs for each geometry: Cube global = 7, Ball global = 5.
% Unique DoFs = active leaf cells * p^3 (marginal-rate approximation, not the
% exact constrained global DoF count).
% MG throughput = unique DoFs / (MG per-cycle time) from the solver=mg run
%   (fixed 20-cycle, un-monitored loop). Solve throughput = unique DoFs /
%   total CG solve time from the solver=cg run at the same problem size; CG
%   iterations is the genuine convergence count from that run.
% p=1 omitted from both geometries; Ball p>=4 and Cube p=5 omitted (no
% completed adaptive=4 run at that size).
\begin{tabular}{llrrrr}
    \toprule
    $p$ & Setting & Unique DoFs   & CG iter. & MG throughput & Solve throughput \\
        &         & (estimate)    &          & [MDoF/s]      & [MDoF/s]         \\
    \midrule
    \multirow{2}{*}{$2$}
        & Cube    & 31\,490\,432  & 9        & 574.2         & 52.3             \\
        & Ball    & 15\,961\,680  & 13       & 108.5         & 7.6              \\
    \midrule
    \multirow{2}{*}{$3$}
        & Cube    & 106\,280\,208 & 9        & 992.3         & 88.8             \\
        & Ball    & 54\,870\,858  & 14       & 244.2         & 15.8             \\
    \midrule
    \multirow{1}{*}{$4$}
        & Cube    & 251\,923\,456 & 10       & 605.9         & 51.8             \\
    \bottomrule
\end{tabular}


==> tables/tab_mg_level_cells.tex <==
% Per-level active-cell counts of the deepest adaptive meshes in the sweep.
% Data: "Per-level cell counts" lines of
%   raw_results/multigrid/sweep_{cube,ball}_adaptive_smooth2.out.
% Cube: global refinement 7 + adaptive refinement 4 (11 levels);
% Ball : global refinement 5 + adaptive refinement 4 ( 9 levels).
% The first levels grow by the uniform factor 2^d = 8 (coarse, global part);
% once the adaptive front sets in the counts grow sub-geometrically and even
% dip (Cube level 7), i.e. the fine levels are small and numerous.
\begin{tabular}{@{}l*{11}{r}@{}}
    \toprule
    Level $\ell$ & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ & $10$ \\
    \midrule
    Cube & 1 & 8 & 64 & 512 & 4\,096 & 32\,768 & 262\,144 & 106\,944 & 385\,536 & 1\,237\,760 & 2\,468\,800 \\
    Ball & 7 & 56 & 448 & 3\,584 & 28\,672 & 69\,712 & 237\,088 & 705\,568 & 1\,277\,440 & & \\
    \bottomrule
\end{tabular}


==> tables/tab_mg_solve_time.tex <==
% Solve-time comparison: DSS multigrid
% Data: raw_results/multigrid/mg_solve_time.csv, generated by
%   raw_results/multigrid/parse_solve_time.py from
%   raw_results/multigrid/sweep_{cube,ball}_perf_smooth2.out (2 smoothing steps).
% For each p, the finest completed solver=mg run (highest REF with a full
% "Total time" summary) is used. Unique DoFs = active leaf cells * p^3
% (marginal-rate approximation, not exact global DoF count).
% MG cycle throughput = unique DoFs / (MG per-cycle time); this comes from
% the MG run (fixed 20-cycle, un-monitored loop -- no real convergence count).
% CG iterations and Solve throughput come from the CG run at the same problem
% size (same REF): CG iterations is the genuine convergence count, and Solve
% throughput = unique DoFs / total CG solve time (the whole solution vector
% over the whole solve, not summed per-iteration throughput).
% p=1 and p=5 Ball omitted: p=1 Ball CG did not converge within the
% 20-iteration cap in this sweep; p=5 Ball has no completed run at all.
\begin{tabular}{llrrrr}
    \toprule
    $p$ & Setting & Unique DoFs   & CG iter. & MG throughput & Solve throughput \\
        &         & (estimate)    &          & [MDoF/s]      & [MDoF/s]         \\
    \midrule
    \multirow{2}{*}{$2$}
        & Cube    & 16\,777\,216  & 8        & 522.1         & 44.7             \\
        & Ball    & 14\,680\,064  & 14       & 108.2         & 7.1              \\
    \midrule
    \multirow{2}{*}{$3$}
        & Cube    & 56\,623\,104  & 9        & 1147.0        & 99.5             \\
        & Ball    & 49\,545\,216  & 15       & 252.6         & 15.4             \\
    \midrule
    \multirow{2}{*}{$4$}
        & Cube    & 134\,217\,728 & 10       & 662.4         & 56.7             \\
        & Ball    & 14\,680\,064  & 14       & 129.6         & 8.5              \\
    \midrule
    $5$ & Cube    & 262\,144\,000 & 11       & 996.5         & 77.0             \\
    \bottomrule
\end{tabular}

